ResNeSt: Split-Attention Networks

It is well known that featuremap attention and multi-path representation are important for visual recognition. In this paper, we present a modularized architecture, which applies the channel-wise attention on different network branches to leverage their success in capturing cross-feature interactions and learning diverse representations. Our design results in a simple and unified computation block, which can be parameterized using only a few variables. Our model, named ResNeSt, outperforms EfficientNet in accuracy and latency trade-off on image classification. In addition, ResNeSt has achieved superior transfer learning results on several public benchmarks serving as the backbone, and has been adopted by the winning entries of COCO-LVIS challenge. The source code for complete system and pretrained models are publicly available.

==> eccv2020kit/tables/res_sota.tex <==


\begin{table}[t]
	\small
	\centering
	\renewcommand\arraystretch{1.1}
	\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
	\resizebox{\linewidth}{!}{
		\begin{tabular}{l|c|c|c|c}
			\toprule[1pt]
			& \multirow{2}{*}{\#P}   &\multirow{2}{*}{GFLOPs} 
			&\multicolumn{2}{c}{top-1 acc (\%)}   \\
			\cline{4-5}
			&&&224$\times$&320$\times$\\
			%\hline\hline
            \cline{1-5}
			ResNet-50~\cite{he2015deep} & 25.5M & 4.14 & 76.15 & 76.86 \\
			ResNeXt-50~\cite{xie2016aggregated} & 25.0M & 4.24  & 77.77 & 78.95  \\
			SENet-50 \cite{hu2017squeeze} & {27.7}M & 4.25 & 78.88 & 80.29   \\
			ResNetD-50~\cite{he2019bag} & 25.6M & 4.34 & 79.15 & 79.70 \\
			SKNet-50 \cite{sknet} & 27.5M  & {4.47} & \secbest 79.21 & \secbest 80.68\\
			ResNeSt-50-fast(\TextRed{\small ours}) & 27.5M & 4.34 & \best 80.64 & \best 81.43 \\ % 80.45* & \best 81.34* 
			\hdashline
			ResNeSt-50(\TextRed{\small ours}) & 27.5M & 5.39 & 81.13 & 81.82  \\
			\hline
			ResNet-101~\cite{he2015deep} & 44.5M & 7.87 & 77.37 & 78.17 \\
			ResNeXt-101~\cite{xie2016aggregated} & 44.3M & 7.99 & 78.89 & 80.14 \\
			SENet-101 \cite{hu2017squeeze} & {49.2}M & 8.00 & 79.42 & 81.39 \\
			ResNetD-101~\cite{he2019bag} & 44.6M & 8.06 & \secbest 80.54 & 81.26 \\
			SKNet-101 \cite{sknet} & 48.9M & {8.46} & {79.81}& \secbest {81.60} \\
			ResNeSt-101-fast(\TextRed{\small ours}) & 48.2M & 8.07 &  \best  81.97 & \best 82.76 \\
			\hdashline
			ResNeSt-101(\TextRed{\small ours}) & 48.3M & 10.2 & 82.27 & 83.00\\
			\bottomrule[1pt]
		\end{tabular}
		% 51.194878 throughput 
		% resnet269_v1f_bicubic train@320 
        % eval @320 0.16154000000000002
        % eval @352 0.15783999999999998
        % eval @384 0.15625999999999995
        % eval @400 0.15603999999999996
        % eval @416 0.15461999999999998
        % eval @448 0.15605999999999998 
        % s3://dist-resnet/results/resnet269_v1f_syncbn_2_bicubic
        
        
	}
	\vspace{1em}
	\caption{Image classification results on ImageNet, comparing our proposed ResNeSt with other ResNet variants of similar complexity in 50-layer and 101-layer configurations. We report top-1 accuracy using crop sizes $224$ and $320$. 
	}
	\label{tab:res_sota}
	\vspace{-2em}
\end{table}


==> everyshi.tex <==
%%
%% This is file `everyshi.sty',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% everyshi.dtx  (with options: `package')
%% 
%% Copyright (C) [1994..1999] by Martin Schroeder. All rights reserved.
%% 
%% This file is part of the EveryShi package
%% 
%% This program may be redistributed and/or modified under the terms
%% of the LaTeX Project Public License, either version 1.0 of this
%% license, or (at your option) any later version.
%% The latest version of this license is in
%%    CTAN:macros/latex/base/lppl.txt.
%% 
%% Happy users are requested to send me a postcard. :-)
%% 
%% The EveryShi package contains these files:
%% 
%%       everyshi.asc
%%       everyshi.dtx
%%       everyshi.dvi
%%       everyshi.ins
%%       everyshi.bug
%% 
%% Error Reports in case of UNCHANGED versions to
%% 
%%                         Martin Schr"oder
%%                         Cr"usemannallee 3
%%                         D-28213 Bremen
%%                         Martin.Schroeder@ACM.org
%% 
%% File: everyshi.dtx Copyright (C) 2001 Martin Schr\"oder
\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{everyshi}
         [2001/05/15 v3.00 EveryShipout Package (MS)]
%% \CharacterTable
%% {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%  Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%  Digits        \0\1\2\3\4\5\6\7\8\9
%%  Exclamation   \!     Double quote  \"     Hash (number) \#
%%  Dollar        \$     Percent       \%     Ampersand     \&
%%  Acute accent  \'     Left paren    \(     Right paren   \)
%%  Asterisk      \*     Plus          \+     Comma         \,
%%  Minus         \-     Point         \.     Solidus       \/
%%  Colon         \:     Semicolon     \;     Less than     \<
%%  Equals        \=     Greater than  \>     Question mark \?
%%  Commercial at \@     Left bracket  \[     Backslash     \\
%%  Right bracket \]     Circumflex    \^     Underscore    \_
%%  Grave accent  \`     Left brace    \{     Vertical bar  \|
%%  Right brace   \}     Tilde         \~}
%%
%% \iffalse meta-comment
%% ===================================================================
%%  @LaTeX-package-file{
%%     author          = {Martin Schr\"oder},
%%     version         = "3.00",
%%     date            = "15 May 2001",
%%     filename        = "everyshi.sty",
%%     address         = {Martin Schr\"oder
%%                        Cr\"usemannallee 3
%%                        28213 Bremen
%%                        Germany},
%%     telephone       = "+49-421-2239425",
%%     email           = "martin@oneiros.de",
%%     pgp-Key         = "2048 bit / KeyID 292814E5",
%%     pgp-fingerprint = "7E86 6EC8 97FA 2995 82C3  FEA5 2719 090E",
%%     docstring       = "LaTeX package which provides hooks into
%%                        \cs{shipout}.
%%  }
%% ===================================================================
%% \fi

\newcommand{\@EveryShipout@Hook}{}
\newcommand{\@EveryShipout@AtNextHook}{}
\newcommand*{\EveryShipout}[1]
   {\g@addto@macro\@EveryShipout@Hook{#1}}
\newcommand*{\AtNextShipout}[1]
   {\g@addto@macro\@EveryShipout@AtNextHook{#1}}
\newcommand{\@EveryShipout@Shipout}{%
   \afterassignment\@EveryShipout@Test
   \global\setbox\@cclv= %
   }
\newcommand{\@EveryShipout@Test}{%
   \ifvoid\@cclv\relax
      \aftergroup\@EveryShipout@Output
   \else
      \@EveryShipout@Output
   \fi%
   }
\newcommand{\@EveryShipout@Output}{%
   \@EveryShipout@Hook%
   \@EveryShipout@AtNextHook%
      \gdef\@EveryShipout@AtNextHook{}%
   \@EveryShipout@Org@Shipout\box\@cclv%
   }
\newcommand{\@EveryShipout@Org@Shipout}{}
\newcommand*{\@EveryShipout@Init}{%
   \message{ABD: EveryShipout initializing macros}%
   \let\@EveryShipout@Org@Shipout\shipout
   \let\shipout\@EveryShipout@Shipout
   }
\AtBeginDocument{\@EveryShipout@Init}
\endinput
%%
%% End of file `everyshi.sty'.

